One-Loop Helicity Amplitudes for ttbar Production at Hadron Colliders

We present compact analytic expressions for all one-loop helicity amplitudes contributing to ttbar production at hadron colliders. Using recently developed generalised unitarity methods and a traditional Feynman based approach we produce a fast and flexible implementation.

==> amp/A1Hpppp.tex <==
\begin{align}
 \begin{split}
	 -i&\ampnorm A_4^{[H]} \left(1_t^{+},2^{+},3^{+},4_\tb^{+} \right) = \\
% 
& - \frac{2 m ( \A{\eta_1}{\eta_4} \AB{2}{1}{2} - \A{2}{\eta_1} \A{3}{\eta_4} \B{2}{3})}{\A{2}{3}^3 \B{2}{3}} \times
    \bigg( s_{23} \, m_H^2 I_{3;1|23|4}^{m_H} 
      + 2 m_H^2 F_{2;23}^{m_H} + \frac{1}{6} s_{23} \bigg) \\ 
 \end{split}
\end{align}


==> amp/A1fpppp.tex <==
-i A & ^{[H]} \left(1_t^+,2^+,3^+,4_\tb^+ \right) = \\
% 
& - \frac{2 m( \A{\eta_1}{\eta_4} \AB{2}{1}{2} - \A{2}{\eta_1} \A{3}{\eta_4} \B{2}{3})}{\A{2}{3}^3 \B{2}{3}} \\ & 
    \bigg( s_{23} \, m_H^2 I_3\left(0,0,s_{23},m_H^2,m_H^2,m_H^2\right) 
      + 2 m_H^2 F_2\left(s_{23},m_H^2,m_H^2\right) + 8 m_H^2 + \frac{1}{3}s_{23} \bigg) \\ 
% 
& + \frac{4 i}{3} A^{(0)}_4(1_t^+,2^+,3^+,4_\tb^+) \, I_2(0,m_H^2,m_H^2)


==> amp/A1qqHppmp.tex <==
\begin{align}
 \begin{split}
  -i\ampnorm A_4 & ^{[H]} \left(1_t^{+},2_\qb^{+},3_q^{-},4_\tb^{+} \right) =  \\
&  \frac{2 }{3 s_{23}} A_4^{(0)} \left(1^{+},2^{+},3^{-},4^{+} \right) \times 
    \left( (2 m_H^2 + s_{23}) \, F_{2;23}^{m_H} + s_{23} I_{2;m_H}^{m_H} + \frac{1}{3} s_{23} \right)
 \end{split}
\end{align}



==> amp/A1slcppmp.tex <==
A^{[slc]} & \left(1^{+},2^{+},3^{-},4^{+} \right)=\\
%
& + I_4\left(s_{12},s_{23},0,m^2,m^2,0,0,0,m^2,0 \right) \bigg( - m \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2 + \frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} + \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{3 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m^3 \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} - \frac{m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^3} - \frac{m^3 \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} - \frac{m^5 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2}\bigg)\\
%
& + I_4\left(s_{13},s_{23},0,m^2,m^2,0,0,0,m^2,0 \right) \bigg( - m \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2 - \frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{3 m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^4 \B{2}{3}^4}{2 \AB{2}{1}{3}^2} + \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}}{2 \AB{2}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} - \frac{m \A{2}{\eta_1} \A{2}{3}^4 \A{2}{\eta_4} \B{2}{3}^5}{2 \AB{2}{1}{3}^3} + \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{\AB{2}{1}{3}^2} + \frac{m^3 \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} - \frac{m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^3} - \frac{m^3 \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{\AB{2}{1}{3}^3} - \frac{m^5 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2}\bigg)\\
%
& + I_4\left(s_{12},s_{13},m^2,0,m^2,0,0,m^2,m^2,0 \right) \bigg(\frac{3 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 \AB{2}{1}{3}} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{5 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{2 \A{2}{3}} + \frac{m^3 \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}} + \frac{3 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} - \frac{3 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{2 \A{2}{3} \AB{2}{1}{3}} + \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\AB{2}{1}{3}} - \frac{3 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{5 m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{3 m^5 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{3 m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} - \frac{3 m^5 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} - \frac{2 m^7 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{m^7 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3} + cont\bigg( - m \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2 + m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}\bigg)\bigg)\\
%
& + I_4\left(s_{12},s_{23},m^2,0,0,m^2,0,m^2,m^2,m^2 \right) \bigg( - m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \AB{2}{1}{2} \B{2}{3}^3}{\AB{2}{1}{3}^2} + \frac{3 m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}}{2 \AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} + \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\AB{2}{1}{3}} + \frac{4 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{6 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{\AB{2}{1}{3}^2} - \frac{3 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3}} + \frac{9 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{2 m^3 \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}} - \frac{6 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{4 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3}} - \frac{7 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{8 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{7 m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} + \frac{3 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{7 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^3} + \frac{m^3 \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} + \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\AB{2}{1}{3}} - \frac{8 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{5 m^5 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{5 m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}} + \frac{8 m^5 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{5 m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{6 m^5 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{6 m^5 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^3} + \frac{3 m^5 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} - \frac{4 m^7 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{4 m^7 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3}\bigg)\\
%
& + int131 \bigg( - m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3} + 10 \frac{\A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} m^3 - 14 \frac{\A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^2} m^5 + \frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{3 m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^4 \B{2}{3}^4}{2 \AB{2}{1}{3}^2} - \frac{3 m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}} + \frac{3 m \A{3}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{2 \AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}} + \frac{m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{3 m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{3 m \A{2}{\eta_1} \A{2}{3}^3 \A{3}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^2} - \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} + \frac{m \A{2}{\eta_1} \A{2}{3}^4 \A{2}{\eta_4} \B{2}{3}^5}{2 \AB{2}{1}{3}^3} + \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\AB{2}{1}{3}} - \frac{4 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{2 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{5 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{3 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3}} - \frac{9 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{13 m^3 \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}} - \frac{4 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3}} + \frac{7 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{8 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{7 m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{19 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{7 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{2 \AB{2}{1}{3}^3} + \frac{4 m^3 \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{\AB{2}{1}{3}^3} + \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\AB{2}{1}{3}} + \frac{m^5 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{5 m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}} + \frac{8 m^5 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{5 m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{6 m^5 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^3} + \frac{9 m^5 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} - \frac{4 m^7 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{4 m^7 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3}\bigg)\\
%
& + I_3\left(0,0,s_{23},0,0,0 \right) \bigg( - \frac{2 m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} + \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3}\bigg)\\
%
& + I_3\left(s_{12},0,m^2,m^2,0,0 \right) \bigg(\frac{m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3}} + \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3}} + \frac{2 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{7 m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{2 \AB{2}{1}{3}} - \frac{9 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}} + \frac{5 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}} - \frac{3 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{7 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}^2} - \frac{m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^3} - \frac{m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} - \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\AB{2}{1}{3}^2} - \frac{7 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{3 m^5 \A{2}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^3}\bigg)\\
%
& + I_3\left(s_{13},0,m^2,m^2,0,0 \right) \bigg( - \frac{m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\AB{2}{1}{3}} + \frac{2 m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{\AB{2}{1}{3}^2} - \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3}} - \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3}} - \frac{2 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{\AB{2}{1}{3}^3} - \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{\AB{2}{1}{3}^3} + \frac{m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{2 \AB{2}{1}{3}} + \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{2 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{7 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{2 \AB{2}{1}{3}} - \frac{5 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}} + \frac{3 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{7 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}^2} - \frac{7 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^3} - \frac{2 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\AB{2}{1}{3}^2} - \frac{5 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{2 \AB{2}{1}{3}^2} - \frac{3 m^5 \A{2}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^3} + \frac{m^5 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3}\bigg)\\
%
& + I_3\left(s_{23},m^2,m^2,0,0,m^2 \right) \bigg( - \frac{m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\beta^{2} \AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\beta^{2} \A{2}{3}} - \frac{m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3}} - \frac{m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}} - \frac{2 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{2 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\beta^{2} \A{2}{3} \AB{2}{1}{3}} + \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\beta^{2} \A{2}{3} \AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} - \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\beta^{2} \AB{2}{1}{3}} - \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\AB{2}{1}{3}} + \frac{2 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{2 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{2 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}} + \frac{4 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\beta^{2} \A{2}{3} \AB{2}{1}{3}} - \frac{4 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{2 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{2 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{2 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{4 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{\AB{2}{1}{3}^2}\bigg)\\
%
& + I_3\left(s_{12},0,m^2,0,m^2,m^2 \right) \bigg(\frac{\A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2}^2 \B{2}{3}}{2 m \AB{2}{1}{2}} + \frac{\A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 m \AB{2}{1}{3}} - \frac{\A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{3}{1}{2} \B{2}{3}^2}{2 m \AB{2}{1}{3}} - \frac{2 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}}{m \AB{2}{1}{2}} - \frac{2 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{m \AB{2}{1}{3}} + \frac{2 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{m \AB{2}{1}{3}} + \frac{2 m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\AB{2}{1}{3}} + \frac{2 m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{2} \AB{2}{1}{3}} - \frac{2 m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{2 m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3}} + \frac{2 m \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} - \frac{5 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{2 \A{2}{3} \AB{2}{1}{3}} - \frac{7 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^3}{2 s_{23} \A{2}{3} \AB{2}{1}{2}} - \frac{2 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{7 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}^2}{2 s_{23} \A{2}{3} \AB{2}{1}{3}} + \frac{2 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{2} \AB{2}{1}{3}} + \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{6 m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\AB{2}{1}{3}} + \frac{3 m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2}{2 s_{23} \AB{2}{1}{2}} + \frac{3 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 s_{23} \AB{2}{1}{3}} - \frac{13 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} - \frac{2 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{2 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}} + \frac{5 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}} - \frac{5 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{17 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} - \frac{5 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{7 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{2 \A{2}{3} \AB{2}{1}{2} \AB{2}{1}{3}} - \frac{5 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}^2} + \frac{3 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{5 m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^3} + \frac{m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{3 m^5 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{2 \AB{2}{1}{2} \AB{2}{1}{3}} - \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\AB{2}{1}{3}^2} - \frac{9 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{5 m^5 \A{2}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{3 m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^3} + \frac{4 m^5 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3}\bigg)\\
%
& + I_3\left(s_{13},0,m^2,0,m^2,m^2 \right) \bigg( - \frac{m \A{2}{\eta_4} \AB{3}{1}{2}^2 \AA{\eta_1}{1 4}{2}}{2 \A{2}{3} \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{m \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \AA{\eta_1}{1 4}{2}}{2 \A{2}{3} \AB{2}{1}{3}^2} + \frac{3 m \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2}{2 \AB{3}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 \AB{2}{1}{3}} - \frac{2 m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{\AB{2}{1}{3}^2} - \frac{2 m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3}} - \frac{2 m \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} + \frac{2 m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}} + \frac{6 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}^2}{2 \A{2}{3} \AB{3}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}} + \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}}{2 \AB{2}{1}{3} \AB{3}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^3}{s_{23} \A{2}{3} \AB{3}{1}{3}} + \frac{5 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}^2}{s_{23} \A{2}{3} \AB{2}{1}{3}} + \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{3 m \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^2} - \frac{m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{\AB{2}{1}{3}^3} + \frac{m^3 \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3} \AA{\eta_1}{1 4}{2}}{2 \AB{2}{1}{3}^3} - \frac{m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{2 \AB{2}{1}{3}} + \frac{m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2}{2 s_{23} \AB{3}{1}{3}} - \frac{m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 s_{23} \AB{2}{1}{3}} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3} \AB{3}{1}{3}} - \frac{5 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{3 m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{9 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{2 \AB{2}{1}{3}} - \frac{5 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}} + \frac{5 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3} \AB{3}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}^2}{s_{23} \A{2}{3} \AB{3}{1}{3}} + \frac{9 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{s_{23} \A{2}{3} \AB{2}{1}{3}} - \frac{15 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{5 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{2 \A{2}{3} \AB{2}{1}{3}^2} - \frac{23 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2 \AB{3}{1}{3}} - \frac{5 m^3 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^3} + \frac{6 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{m^5 \A{2}{\eta_4} \B{2}{3} \AA{\eta_1}{1 4}{2}}{2 \AB{2}{1}{3}^3} + \frac{m^5 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{2 \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\AB{2}{1}{3}^2} - \frac{2 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{9 m^5 \A{2}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{2 \AB{2}{1}{3}^2} + \frac{m^5 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}^2 \AB{3}{1}{3}} - \frac{3 m^5 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^3} + \frac{7 m^5 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3} - \frac{m^7 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}}{2 \AB{2}{1}{3}^3}\bigg)\\
%
& + I_3\left(s_{23},m^2,m^2,m^2,m^2,0 \right) \bigg(\frac{\A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2}^2 \B{2}{3}}{2 m \AB{3}{1}{3}} - \frac{\A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{2 m \AB{2}{1}{3}} - \frac{3 \A{\eta_1}{\eta_4} \A{2}{3}^3 \AB{3}{1}{2} \B{2}{3}^3}{2 m \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{3 \A{\eta_1}{\eta_4} \A{2}{3}^3 \AB{2}{1}{2} \B{2}{3}^3}{2 m \AB{2}{1}{3}^2} + \frac{3 \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 m \AB{3}{1}{3}} - \frac{3 \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{2 m \AB{2}{1}{3}} - \frac{2 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}}{m \AB{3}{1}{3}} + \frac{2 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}}{m \AB{2}{1}{3}} - \frac{\A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2}^2 \B{2}{3}^2}{m \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{\A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} cont\bigg(m^ - 1\bigg) + \frac{3 \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}^3}{2 m \AB{2}{1}{3} \AB{3}{1}{3}} - \frac{3 \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^3}{2 m \AB{2}{1}{3}^2} - \frac{m \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2}{\AB{3}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\AB{2}{1}{3}} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{3 m \A{\eta_1}{\eta_4} \A{2}{3}^4 \B{2}{3}^4}{2 \AB{2}{1}{3}^2 \AB{3}{1}{3}} - \frac{m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}} - \frac{3 m \A{3}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{2 \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{2 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{3}{1}{3}} - \frac{2 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\A{2}{3} \AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^3}{s_{23} \A{2}{3} \AB{3}{1}{3}} + \frac{3 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}^2}{s_{23} \A{2}{3} \AB{2}{1}{3}} + \frac{2 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3} \AB{3}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} + \frac{m \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^3}{\AB{2}{1}{3}^2 \AB{3}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{2}{3}^3 \A{3}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^2 \AB{3}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} + \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2}{s_{23} \AB{3}{1}{3}} + \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{3}{1}{2}^2}{s_{23} \AB{2}{1}{2}} + \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3} \AB{3}{1}{3}} + \frac{6 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^2 \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{m^3 \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{2 \AB{2}{1}{3}^2 \AB{3}{1}{3}} - \frac{4 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}} - \frac{2 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3} \AB{3}{1}{3}} - \frac{12 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{6 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{3 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\A{2}{3} \AB{2}{1}{3} \AB{3}{1}{3}} + \frac{6 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{4 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\AB{2}{1}{3} \AB{3}{1}{3}} + \frac{2 m^5 \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\AB{2}{1}{2} \AB{2}{1}{3}} + \frac{4 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{8 m^5 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3}\bigg)\\
%
& + I_3\left(0,0,s_{23},m^2,m^2,m^2 \right) \bigg(\frac{m \A{\eta_1}{\eta_4} \A{2}{3} \AB{3}{1}{2} \B{2}{3}}{2 \AB{2}{1}{3}} + \frac{3 m \A{\eta_1}{\eta_4} \A{2}{3}^2 \AB{2}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} - \frac{m \A{\eta_1}{\eta_4} \A{2}{3}^3 \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{2 m \A{3}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}} - \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{\AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}^2}{2 \AB{2}{1}{3}^2} + \frac{3 m \A{2}{\eta_1} \A{2}{3}^2 \A{3}{\eta_4} \B{2}{3}^3}{2 \AB{2}{1}{3}^2} - \frac{m \A{2}{\eta_1} \A{2}{3}^3 \A{2}{\eta_4} \B{2}{3}^4}{2 \AB{2}{1}{3}^3} + \frac{4 m^3 \A{\eta_1}{\eta_4} \A{2}{3} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{5 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}}{\AB{2}{1}{3}} - \frac{8 m^3 \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{3 m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{4 m^3 \A{2}{\eta_1} \A{2}{3} \A{3}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^2} - \frac{3 m^3 \A{2}{\eta_1} \A{2}{3}^2 \A{2}{\eta_4} \B{2}{3}^3}{\AB{2}{1}{3}^3} + \frac{4 m^5 \A{\eta_1}{\eta_4} \A{2}{3} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{4 m^5 \A{2}{\eta_1} \A{2}{3} \A{2}{\eta_4} \B{2}{3}^2}{\AB{2}{1}{3}^3}\bigg)\\
%
& + I_2\left(s_{23},0,0 \right) \bigg( - \frac{m \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\beta^{2} \AB{2}{1}{3}} - \frac{2 m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\beta^{2} s_{23} \AB{2}{1}{3}} + \frac{2 m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\beta^{2} s_{23} \A{2}{3}} + \frac{2 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\beta^{2} \A{2}{3} \AB{2}{1}{3}} + \frac{4 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\beta^{2} s_{23} \A{2}{3} \AB{2}{1}{3}} - \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} - \frac{2 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\beta^{2} s_{23} \A{2}{3} \AB{2}{1}{3}}\bigg)\\
%
& + I_2\left(s_{23},m^2,m^2 \right) \bigg(\frac{m \A{\eta_1}{\eta_4} \AB{3}{1}{2}}{\beta^{2} \AB{2}{1}{3}} + \frac{2 m \A{\eta_1}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\beta^{2} s_{23} \AB{2}{1}{3}} - \frac{2 m \A{3}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\beta^{2} s_{23} \A{2}{3}} - \frac{2 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{3}{1}{2}}{\beta^{2} \A{2}{3} \AB{2}{1}{3}} - \frac{4 m \A{2}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \AB{3}{1}{2}}{\beta^{2} s_{23} \A{2}{3} \AB{2}{1}{3}} + \frac{m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\AB{2}{1}{3}^2} + \frac{2 m \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2}^2}{\beta^{2} s_{23} \A{2}{3} \AB{2}{1}{3}}\bigg)

==> amp/A1slcpppp.tex <==
A^{[slc]} & \left(1^{+},2^{+},3^{+},4^{+} \right)=\\
%
& + I_4\left(s_{12},s_{23},0,m^2,m^2,0,0,0,m^2,0 \right) \bigg(m^3 \A{\eta_1}{\eta_4} \B{2}{3}^2\bigg)\\
%
& + I_4\left(s_{13},s_{23},0,m^2,m^2,0,0,0,m^2,0 \right) \bigg(m^3 \A{\eta_1}{\eta_4} \B{2}{3}^2\bigg)\\
%
& + I_4\left(s_{12},s_{13},m^2,0,m^2,0,0,m^2,m^2,0 \right) \bigg(2 m^3 \A{\eta_1}{\eta_4} \B{2}{3}^2 - \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\A{2}{3}} + \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2}^2}{\A{2}{3}^2} - \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{3} \B{2}{3}}{2 \A{2}{3}^2} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2 \A{2}{3}^2} + \frac{m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{2 \A{2}{3} \AB{3}{1}{2}} - \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{2 \A{2}{3} \AB{2}{1}{3}}\bigg)\\
%
& + I_4\left(s_{12},s_{23},m^2,0,0,m^2,0,m^2,m^2,m^2 \right) \bigg(m^3 \A{\eta_1}{\eta_4} \B{2}{3}^2 + \frac{m^3 \B{2}{3} \AA{\eta_1}{K_{12} K_{23}}{\eta_4}}{\A{2}{3}} + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{2 \A{2}{3} \AB{3}{1}{2}} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{2 \A{2}{3} \AB{2}{1}{3}} + \frac{2 m^5 \A{\eta_1}{\eta_4} \B{2}{3}}{\A{2}{3}} + \frac{m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{3}{1}{2}} - \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{2}{1}{3}}\bigg)\\
%
& + int131 \bigg(m^3 \A{\eta_1}{\eta_4} \B{2}{3}^2 + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^3}{2 \AB{3}{1}{2}} - \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{2 \A{2}{3} \AB{3}{1}{2}} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^3}{2 \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}^2}{2 \A{2}{3} \AB{2}{1}{3}} + \frac{2 m^5 \A{\eta_1}{\eta_4} \B{2}{3}}{\A{2}{3}} + \frac{m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{3}{1}{2}} - \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{2}{1}{3}} + \frac{AA\bigg(e1}{K\bigg(p3,p1},K\bigg(p2,p3\bigg),e4\bigg) m^3 \B{2}{3},\A{2}{3}\bigg)\bigg)\\
%
& + I_3\left(s_{12},0,m^2,m^2,0,0 \right) \bigg(\frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\A{2}{3}^2} + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{3}{1}{2}} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{2}{1}{3}}\bigg)\\
%
& + I_3\left(s_{13},0,m^2,m^2,0,0 \right) \bigg(\frac{2 m^3 \A{\eta_1}{\eta_4} \B{2}{3}}{\A{2}{3}} - \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\A{2}{3}^2} + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{2 \A{2}{3} \AB{3}{1}{2}} - \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{3}{1}{2}} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{2 \A{2}{3} \AB{2}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{2}{1}{3}}\bigg)\\
%
& + I_3\left(s_{12},0,m^2,0,m^2,m^2 \right) \bigg(\frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\A{2}{3}^2} + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{3}{1}{2}} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{2}{1}{3}}\bigg)\\
%
& + I_3\left(s_{13},0,m^2,0,m^2,m^2 \right) \bigg(\frac{2 m^3 \A{\eta_1}{\eta_4} \B{2}{3}}{\A{2}{3}} - \frac{2 m^3 \A{\eta_1}{\eta_4} \AB{2}{1}{2}}{\A{2}{3}^2} + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{2 \A{2}{3} \AB{3}{1}{2}} + \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{3} \B{2}{3}}{\A{2}{3}^2 \AB{3}{1}{3}} - \frac{3 m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{3}{1}{2}} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{2 \A{2}{3} \AB{2}{1}{3}} - \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{2 \A{2}{3}^2 \AB{3}{1}{3}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\A{2}{3}^2 \AB{2}{1}{3}} - \frac{m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{3}{1}{2} \AB{3}{1}{3}} + \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{2 \A{2}{3} \AB{2}{1}{3} \AB{3}{1}{3}}\bigg)\\
%
& + I_3\left(s_{23},m^2,m^2,m^2,m^2,0 \right) \bigg( - \frac{m^3 \B{2}{3} \AA{\eta_1}{K_{12} K_{23}}{\eta_4}}{\A{2}{3} \AB{2}{1}{2}} - \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{3} \B{2}{3}}{\A{2}{3}^2 \AB{2}{1}{2}} - \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\A{2}{3}^2 \AB{3}{1}{2}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{3}{1}{2} \B{2}{3}}{\A{2}{3}^2 \AB{2}{1}{2}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \AB{2}{1}{2} \B{2}{3}}{\A{2}{3}^2 \AB{2}{1}{3}} - \frac{m^5 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{3}{1}{2} \AB{3}{1}{3}} + \frac{m^5 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{2}{1}{3} \AB{3}{1}{3}} - \frac{AA\bigg(e1}{K\bigg(p3,p1},K\bigg(p2,p3\bigg),e4\bigg) m^3 \B{2}{3},\A{2}{3} \AB{3}{1}{3}\bigg)\bigg)\\
%
& + I_3\left(0,0,s_{23},m^2,m^2,m^2 \right) \bigg(\frac{2 m^3 \A{\eta_1}{\eta_4} \B{2}{3}}{\A{2}{3}} - \frac{m^3 \A{3}{\eta_1} \A{3}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{3}{1}{2}} + \frac{m^3 \A{2}{\eta_1} \A{2}{\eta_4} \B{2}{3}^2}{\A{2}{3} \AB{2}{1}{3}}\bigg)
